Few-shot Learning with Multilingual Language Models

Large-scale generative language models such as GPT-3 are competitive few-shot learners. While these models are known to be able to jointly represent many different languages, their training data is dominated by English, potentially limiting their cross-lingual generalization. In this work, we train multilingual generative language models on a corpus covering a diverse set of languages, and study their few- and zero-shot learning capabilities in a wide range of tasks. Our largest model with 7.5 billion parameters sets new state of the art in few-shot learning in more than 20 representative languages, outperforming GPT-3 of comparable size in multilingual commonsense reasoning (with +7.4% absolute accuracy improvement in 0-shot settings and +9.4% in 4-shot settings) and natural language inference (+5.4% in each of 0-shot and 4-shot settings). On the FLORES-101 machine translation benchmark, our model outperforms GPT-3 on 171 out of 182 directions with 32 training examples, while surpassing the official supervised baseline in 45 directions. We conduct an in-depth analysis of different multilingual prompting approaches, showing in particular that strong few-shot learning performance across languages can be achieved via cross-lingual transfer through both templates and demonstration examples. Finally, we evaluate our models in social value tasks such as hate speech detection in five languages and find it has limitations similar to comparable sized GPT-3 models.

==> sections/background.tex <==
\section{Background}

\subsection{Pre-trained Large Language Models}


% Pre-training Language Models on large, unsupervised corpora of texts has been a common practice in the past years. Early work \cite{Mikolov2013EfficientSpace} focused on learning useful representations for individual words, which has later been gradually extended \cite{Peters2018DeepRepresentations} to also incorporate context in a given sentence.

By pre-training a Transformer architecture \cite{Vaswani2017AttentionNeed} on a large corpus of text, BERT \cite{Devlin2018BERT:Understanding} has outperformed state-of-the-art in a wide variety of benchmarks. Numerous variations of this approach have been published since then: RoBERTa \cite{Liu2019RoBERTa:Approach}, T5 \cite{Raffel2019ExploringTransformer}, BART \cite{Lewis2019BART:Comprehension}, Switch Transformers \cite{Fedus2021SwitchSparsity} just to name a few. 

Notably, all of these models require some amount of additional data to fine-tune their parameters to specific tasks. When this additional data is very limited (few-shot learning), prompting-based methods  \cite{Schick2020ExploitingInference} tend to perform particularly well \cite{Scao2021HowWorth}. This line of work formulates various downstream tasks as language modeling problems by asking the model to fill in blanks in sentences . For example, \cite{Petroni2019LanguageBases} constructed such prompts (templates) to extract knowledge from language models. 

% comment{TODO: fix bibtex entry, need to include year} 
% [Daniel] Added a new Mendeley entry, looks better now.

\cite{Jiang2019HowKnow} and \cite{Shin2020AutoPrompt:Prompts} used data mining techniques and gradient based search respectively to find better prompts than manually chosen ones and \cite{Schick2020AutomaticallyClassification} found better tokens to represent labels of classification tasks. As opposed to these discrete prompting approaches, \cite{Li2021Prefix-Tuning:Generation}, \cite{Qin2021LearningPrompts}, \cite{Liu2021GPTToo} go one step further and searches for good "prompts" in the continuous space, this is often referred to as soft prompting.

While most work discussed in this Section is focused on English, there is extensive research on multilingual adaptations of these models - this is discussed in Section \ref{section:related_work}.

\subsection{In-Context Learning}

\citet{Brown2020LanguageLearners} provide a few examples of solved tasks as part of the context (prompt) for an extremely large, pre-trained language model, GPT-3. This method, commonly referred to as "in-context" learning, removes the need for any task-specific updates to the model parameters: the few-shot examples that one would normally use for fine-tuning are provided at inference time to the very same model for each task. In-context learning capabilities of language models only emerge at scale, when a model has sufficiently many parameters. \cite{Wei2021FINETUNEDLEARNERS} shows that such pre-trained language models can also be further fine-tuned to work with prompts better. 

As seen in Section \ref{section:related_work}, the multilingual aspect of in-context learning has not been studied as extensively as it had been the case for previous families of models.

==> tables/multi_few_shot_scaling_resource_level.tex <==
\begin{table*}[t]
\centering
\scalebox{0.66}{
    \begin{tabular}{llllllllllllrrlll}
    \toprule
         & {} & \multicolumn{15}{l}{mean} \\
         & {} & \multicolumn{15}{l}{accuracy::mean} \\
         & pivoting\_task\_group & \multicolumn{10}{l}{Language Modeling} & \multicolumn{5}{l}{NLI} \\
         & pivoting\_task & \multicolumn{4}{l}{storycloze} & \multicolumn{4}{l}{xcopa} & \multicolumn{2}{l}{xwinograd} & \multicolumn{3}{l}{xnli} & \multicolumn{2}{l}{pawsx} \\
         & pivoting\_resource\_level &                hi &   me &   lo & ex-lo &    hi &   me &   lo & ex-lo &        hi &   me &    hi &   me &   lo &    hi &   me \\
    pivoting\_model\_size & nb\_few\_shot\_samples &                   &      &      &       &       &      &      &       &           &      &       &      &      &       &      \\
    \midrule
     564M & 0   &                   &      &      &       &  52.8 & 53.6 & 50.8 &  51.8 &      54.2 & 51.5 &  38.7 & 40.7 & 38.5 &  53.7 & 53.3 \\
         & 4   &              57.8 & 55.2 & 56.8 &  54.0 &  52.9 & 53.2 & 51.6 &  51.4 &      54.4 & 51.5 &  42.2 & 40.8 & 38.8 &  51.8 & 50.4 \\
         & 32  &              57.9 & 55.4 & 56.6 &  53.6 &  53.3 & 53.1 & 51.2 &  51.4 &      55.7 & 52.1 &  39.5 & 37.3 &      &  52.8 & 52.5 \\
    1.7B & 0   &              61.8 & 59.8 & 58.9 &  56.4 &  55.9 & 57.9 & 55.2 &  52.6 &      55.3 & 52.8 &  43.3 & 43.8 & 42.1 &  53.0 & 53.4 \\
         & 1   &              61.6 & 60.4 & 58.7 &  56.1 &       &      &      &       &           &      &  44.3 & 42.4 & 40.7 &       &      \\
         & 4   &              62.0 & 60.7 & 58.7 &  56.5 &  58.8 & 57.8 & 55.6 &  52.3 &      57.0 & 54.2 &  45.2 & 44.3 & 41.1 &  54.3 & 53.2 \\
         & 32  &              62.6 & 61.1 & 59.2 &  56.4 &  59.6 & 58.4 & 55.4 &  50.9 &      59.1 & 53.9 &  42.1 & 40.8 &      &  53.8 & 54.4 \\
         & 128 &                   &      &      &       &  60.0 & 58.5 & 55.9 &  50.5 &      58.9 & 54.9 &  41.1 & 39.7 &      &  53.5 & 54.0 \\
    7.5B & 0   &              67.8 & 65.5 & 63.0 &  60.7 &  61.6 & 60.4 & 58.5 &  52.2 &      60.7 & 57.5 &  47.0 & 46.5 & 43.7 &  56.1 & 50.8 \\
         & 1   &              68.1 & 65.8 & 63.3 &  60.6 &  65.3 & 61.1 & 59.8 &  52.8 &      61.5 & 57.9 &  43.8 & 42.3 & 39.7 &  53.5 & 53.5 \\
         & 4   &              69.0 & 66.7 & 64.1 &  61.2 &  68.2 & 63.8 & 61.7 &  53.0 &      62.7 & 58.7 &  48.2 & 47.5 & 44.0 &  54.4 & 53.5 \\
         & 32  &              69.3 & 67.1 & 64.6 &  61.1 &  69.2 & 65.4 & 62.7 &  54.5 &      66.5 & 58.7 &  46.9 & 46.6 & 46.3 &  54.3 & 53.7 \\
         & 128 &                   &      &      &       &  68.7 & 65.8 & 61.9 &  54.1 &      65.2 & 58.7 &  45.6 & 45.2 & 46.2 &  54.3 & 54.3 \\
    \bottomrule
    \end{tabular}
}
\caption{Few-shot performance w.r.t. model scaling broken down by language resource level. \vic{Add std across resource levels.}}
\end{table*}

==> tables/xcopa.tex <==


\begin{table*}[t!]
    \centering
    \scalebox{0.68}{
        \begin{tabular}{ll|r|rrrrr|rrr|rr|c}
        \toprule
             % & {} & \multicolumn{11}{l}{accuracy::mean} \\
             &  & \multicolumn{1}{c|}{high} & \multicolumn{5}{c}{medium} & \multicolumn{3}{c}{low} & \multicolumn{2}{c}{ex-low} & Avg. \\
            model & \#\ shot &           zh &   id &       it &   th &   tr &   vi &   et &   sw &   ta &            ht &   qu &  \\
        \midrule
         
        \model{GPT-3}{6.7B} & 0   &  55.0 & 60.2 & \bf 61.6 & 53.6 & 53.4 & 52.8 & 50.8 & 52.2 & 55.0 & 51.8 & \bf 50.0 & 54.2\\
                    & 4   &  57.8 & 60.8 & 64.5  & 54.2 & 52.9 & 54.8 & 51.8 & 52.0 & 54.9 &  51.5 & \bf 49.7 & 55.0 \\
         \midrule
         
        % \model{\Oursns}{6.7B} \textit{EN-only} &   0&	50.4 &	53.2 &	53.2 &	52.2 &	49.4 &	51.4 &	50.6 &	51.8 &	48.0 &	45.6 &	\bf 50.0 & 50.5\\
        %         &   4&	49.5 &	52.4 &	54.2 &	51.2 &	49.4 &	50.9 &	50.0 &	50.8 &	47.4 &	48.3 &	\bf 49.7  & 50.3\\
        % \midrule       
        
        \model{\Oursns}{7.5B} & 0   & \bf 62.4 &   \bf 66.6  &  60.8  & \bf 56.8 & \bf 56.8 & \bf 61.4 & \bf 61.6 & \bf 57.6 & \bf 56.2 &  \bf 57.0 & 47.4 & \bf  58.6 \\
             & 4   & \bf 67.2  & \bf 68.9 & \bf 69.2 & \bf 62.0 & \bf 58.5 & \bf 65.6 & \bf 65.9 & \bf 62.9 & \bf 56.3 &          \bf 58.9 & 47.1 & \bf 62.0\\
             
        \midrule
        \midrule
        Translate+\xlmgen & 0 &	75.0 &	73.2 &	76.0  & 53.8 &	72.4 &	72.2 &	72.4 &	63.8 &	67.2 &	65.0 & -  & 67.4$^\dagger$ \\
        
                            & 4 &	78.5 & 	75.8 &	80.6  & 57.7 &	73.7 &	76.0 &	73.6 &	67.2 &	69.9 &	67.0 & - & 70.0$^\dagger$ \\
        
        
        \bottomrule
        \end{tabular}
    }
    
    % \vic{Is the translate-test baseline average comparable with the other rows given we don't have qu performance? If not, let's explain this in the title.}
    
    % [Daniel] Adddressed this in a footnote.
    
    \caption{Comparison of different models on XCOPA. $^\dagger$Google Translation API is not available for \lang{qu}. For the averaged translate-test results we % used the results without translation ("\Ours 6.7B EN-only" row) 
    directly used the for the "\Ours 6.7B EN-only" model to obtain the \lang{qu} entry.}
    \label{tab:comp_xcopa}
\end{table*}


==> tables/xstorycloze.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.68}{
        \begin{tabular}{ll|rrrr|rr|rrr|rr|c}
        \toprule
            %  & {} & \multicolumn{11}{l}{accuracy::mean} \\
             &  & \multicolumn{4}{c|}{high} & \multicolumn{2}{c|}{medium} & \multicolumn{3}{c|}{low} & \multicolumn{2}{c|}{ex-low} & Avg. \\
        %\midrule
           model & \#\ shot &     en &   es &   ru &   zh &   ar &      id &   hi &     sw &   te &     eu &        my \\
       
        \midrule
       
        \model{GPT-3}{6.7B} & 0  &   73.4 & 62.4 & 56.9 & 55.8 & 48.4 &  56.6    & 50.1 & 49.4 & 52.8 & 51.2 &          49.5 & 55.1 \\
             
             & 4  &          74.4& 62.2 & 56.4 & 54.7 & 47.7 &  55.4    & 49.6 & 49.3 & 52.8 & 51.1 &          49.5 & 54.8 \\
        \midrule  
        
        % \model{\Oursns}{6.7B} \textit{EN-only}  & 0&	\bf 81.2 &	62.4 &	53.7 &	54.0 &	53.1 &	54.5 &	52.8 &	53.9 &	54.5 &	52.3 &	51.3 & 56.7 \\ 
        %                              & 4&	\bf 82.6 &	61.9 &	53.6 &	54.2 &	53.4 &	53.5 &	53.2 &	53.6 &	54.5 &	51.4 &	52.4 & 56.8 \\
        
        % \midrule
        
        \model{\Oursns}{7.5B} & 0  &           75.0 & \bf 68.1 & \bf 71.0 & \bf 66.6 &   \bf 58.3 & \bf 70.1 &  \bf 60.9 &   \bf 65.0 & \bf 61.7 &   \bf 62.3 &       \bf 60.7  & \bf 65.4 \\
            
             & 4  &            75.9 & \bf 69.2 & \bf 72.4 & \bf 67.7 &  \bf 59.8 &  \bf 70.8 &  \bf 62.5 &   \bf 65.2 & \bf 63.4 &     \bf 63.8 &     \bf 61.2 & \bf 66.5 \\
             
        \midrule
        \midrule
        Translate + \xlmgen & 0 & 81.2 & 75.6 &	75.4 &	72.9 &	71.5 &	71.2 &	70.5 &	70.0 &	66.9 &	70.5 &	72.7 & 72.6 \\
                            & 4 & 82.6 & 75.0 &	75.3 &	73.1 &	71.8 &	72.0 &	71.6 &	71.0 &	68.4 &	72.2 &	72.0 & 73.2 \\
             
        \bottomrule
        \end{tabular}
    }
    \caption{Comparison of different models on XStoryCloze.} % \xian{double check: our 6.7B En model outperforms GPT-3 by large margin on En. I've rerun the curie eval on 0-shot and the result stays the same.} }
    
    % Log /checkpoint/xianl/few_shot/multilingual_eval/openai_curie_storycloze_val2016_split_20_80_train_val2016_split_20_80_eval_lang/task.storycloze_tmp.storycloze_train.val2016_split_20_80_train.en_val.None.en_eval.val2016_split_20_80_eval.en_calib.None_fs0_results.json.}
    
    %[Daniel] /checkpoint/danielsimig/multilingual/en_6.7B/storycloze_6.7B_gpt3_setting_fs.0_t5_smpl.All_current/task.storycloze_tmp.storycloze_train.val2016_split_20_80_train.en_val.None.en_eval.val2016_split_20_80_eval.en_calib.None_fs0_results.json
    % max_tokens seems to be 2048 in both cases.
    
     \label{tab:comp_xstorycloze}
\end{table*}

